Rethinking State Management in Actor Systems for Cloud-Native Applications

The actor model has gained increasing popularity. However, it lacks support for complex state management tasks, such as enforcing foreign key constraints and ensuring data replication consistency across actors. These are crucial properties in partitioned application designs, such as microservices. To fill this gap, we start by analyzing the key impediments in state-of-the-art actor systems. We find it difficult for developers to express complex data relationships across actors and reason about the impact of state updates on performance due to opaque state management abstractions. To solve this conundrum, we develop SmSa, a novel data management layer for actor systems, allowing developers to declare data dependencies that cut across actors, including foreign keys, data replications, and other dependencies. SmSa can transparently enforce the declared dependencies, reducing the burden on developers. Furthermore, SmSa employs novel logging and concurrency control algorithms to support transactional maintenance of data dependencies. We demonstrate SmSa can support core data management tasks where dependencies across components appear frequently without jeopardizing application logic expressiveness and performance. Our experiments show SmSa significantly reduces the logging overhead and leads to increased concurrency level, improving by up to 2X the performance of state-of-the-art deterministic scheduling approaches. As a result, SmSa will make it easier to design and implement highly partitioned and distributed applications.

==> 02_background.tex <==
\section{Background}

\subsection{Orleans}
Orleans~\cite{Orleans} is a framework that facilitates the development of distributed applications through virtual actors~\cite{Bernstein2014}. Orleans automatically allocates virtual actors in available nodes and deactivates actors when they are no longer needed. In addition, Orleans transparently migrates virtual actors from faulty computational resources to others in case of failures, ensuring that the application remains functional.

To aid developers in designing data-intensive applications, Orleans recently introduced state management and transaction management APIs~\cite{OrleansTxn} (\texttt{OrleansTxn}). Through transactional objects modeled as the state of actors~\cite{tx_state}, Orleans can preclude developers from explicitly implementing transactional guarantees. \texttt{OrleansTxn} adopts a locking-based concurrency control method and applies Early-Lock Release for approaching a higher level of concurrency. However, as reported by recent research \cite{Snapper, Marketplace}, \texttt{OrleansTxn} is vulnerable to contentions, often leading to low performance. 

\subsection{\texttt{Snapper}}
\texttt{Snapper}~\cite{Snapper} is an actor transaction library designed to enhance the performance of multi-actor transactions meanwhile preserving the ACID transactional properties. \texttt{Snapper} leverages deterministic scheduling for PACT, a type of transaction that declares the actor access information when it is submitted to the system. Based on this pre-declared information, \texttt{Snapper} employs a group of coordinator actors to generate deterministic transaction execution schedules for every batch of PACTs. Each such schedule consists of a sequence of PACTs that are relevant to a particular actor. Afterward, \texttt{Snapper} delivers such batch schedules to corresponding actors via asynchronous messages. Each actor is supposed to execute transactional invocations of PACTs individually in the pre-determined order. Under the PACT execution, transactions are scheduled, executed, committed, and logged all at the batch level.

In addition to deterministic execution, \texttt{Snapper} also supports conventional non-deterministic strategies, such as Strict Two-Phase Locking (S2PL) and Two-Phase Commit (2PC), for transactions whose actor access information cannot be pre-declared. This type of transaction is called ACT. Another standout feature of Snapper is its ability to execute concurrent hybrid workloads, wherein some transactions are executed deterministically while others follow non-deterministic methods. This hybrid execution model maximizes the advantages of deterministic execution, which can achieve high transaction throughput while maintaining flexibility for non-deterministic workloads.

% \subsection{Actor State Management}
Although devising novel deterministic concurrency control algorithms to actor systems, \texttt{Snapper} still inherits the same expressiveness impediments found in Orleans. %In both systems, developers must reason about the trade-offs of different transactional object designs. On one side, managing multiple transactional objects (e.g., one per entity) provides a finer-grained state manipulation. However, it can increase the concurrency control overhead since more objects must be tracked to ensure transactional isolation. On the other hand, modelling a single transactional object can incur higher I/O costs since all entities encapsulated by the object are necessarily offloaded to storage to ensure durability. As the transactional object size tends to increase over time, that can severely impact the application performance at some point. Other actor frameworks follow a similar approach to modelling durable states~\cite{Akka}. Unfortunately, these actor and state modelling performance trade-offs are not always crystal clear for developers~\cite{Wang2019}.

For instance, developers 
find no appropriate abstractions to model complex relationships across actors and fall prey to error-prone implementations to fulfil key properties that arise in real-world distributed applications~\cite{vldb2021}.

This work is the first to focus on advancing the existing opaque actor state management abstraction, allowing developers to express complex relationships across actors and benefit from data integrity enforcement.

% In actor systems, though, by having no way to express these properties, developers must map  relationships across actors explicitly (e.g., which carts contain a certain product) and ensure their correctness in application code. Besides being complex and error-prone, such encoding is oblivious to transaction management, leading to isolation anomalies. Therefore, an opaque state management abstraction limits the ability of developers to express important safety properties that arise in data-intensive applications.


% rich state management abstraction



\subsection{Key Partitioning Algorithm}
Data partitioning is a fundamental mechanism applied in distributed systems to balance workload, reduce costly data transfer, improve performance, and achieve scalability. An effective partitioning strategy ensures that the data is distributed evenly and similar keys can be accessed quickly and efficiently. Additionally, in many cases, different types of data are accessed or combined together, such as the $join$ operation in database systems. Thus, it is crucial to support the co-partition of multiple tables on one actor. 

However, the effectiveness of key partitioning largely depends on how well it aligns with the specific requirements and access patterns of the application. Besides, plenty of research works have discussed the principles of partitioning data and how to model an application to actors \cite{Wang2019}. Therefore, in \texttt{SmSa}, we rely on developers to devise and implement partitioning algorithms tailored specifically to their use cases.



\subsection{Key-Value Store}
This kind of semi-structured data is supported in plenty of NoSQL database systems \cite{} but has not been adopted for maintaining key relations. 

However, this concept has rarely been discussed in the context of key-value stores or actor systems \cite{}, whilst dependencies between different data records exist in an extensive range of applications that are built on key-value or actor models. For example, ... \cite{}.

A common concern when introducing relationships between keys to a key-value store is its need for table schemes. A relational database system declares a table with a particular set of attributes or columns; each can be a foreign key to another table. In a key-value store, the value part of a record has no such scheme. The simplicity of the key-value data model is the primary trick to allow fast data access. Another well-recognised challenge is to enforce referential integrity and maintain dependencies between keys, which violate the implicit horizontal scalability aimed by a key-value store. To enable key relations or references, existing solutions either 
resort to a back-end relational database system or put the burden on developers to enforce constraints in the application code.
